Learning with less data via Weakly Labeled Patch Classification in Digital Pathology

In Digital Pathology (DP), labeled data is generally very scarce due to the requirement that medical experts provide annotations. We address this issue by learning transferable features from weakly labeled data, which are collected from various parts of the body and are organized by non-medical experts. In this paper, we show that features learned from such weakly labeled datasets are indeed transferable and allow us to achieve highly competitive patch classification results on the colorectal cancer (CRC) dataset [1] and the PatchCamelyon (PCam) dataset [2] while using an order of magnitude less labeled data.

==> extra.tex <==
%%%%
\begin{figure}[H]
\centering
{\setlength{\tabcolsep}{2pt}
\scalebox{0.64}{ %0.64
\fbox{
\begin{tabular}{cc!{\vrule width 5pt}ccc}
&
\textbf{Query} & \textbf{Rank 1} & \textbf{Rank 2} & \textbf{Rank 3}\\
\parbox[t]{3mm}{\multirow{1}{*}{\rotatebox[x=-10in]{90}{\vspace{10pt}Tumour Epithelium\hspace{-65pt}}}}&
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/36_0_0.png}\ \ \ &
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/36_1_2.png}&
\includegraphics[width=1.0in,height=1.0in, cfbox=green 3pt]{figs/colon_ret/36_3_0.png}&
\includegraphics[width=1.0in,height=1.0in, cfbox=green 3pt]{figs/colon_ret/36_3_0.png} \\
%Tumour Epithelium & & & \\
\parbox[t]{2mm}{\multirow{1}{*}{\rotatebox[x=-10in]{90}{\vspace{10pt}Simple Stroma\hspace{-60pt}}}}&
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/7_0_1.png}&
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/7_1_2.png}&
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/7_2_2.png}&
\includegraphics[width=1.0in,height=1.0in, cfbox=green 3pt]{figs/colon_ret/7_3_1.png} \\
%Simple Stroma & & & \\
\parbox[t]{2mm}{\multirow{1}{*}{\rotatebox[x=-10in]{90}{\vspace{10pt}Complex Stroma\hspace{-60pt}}}}&
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/1_0_2.png}&
\includegraphics[width=1.0in,height=1.0in, cfbox=green 3pt]{figs/colon_ret/1_1_2.png}&
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/1_2_3.png}&
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/1_3_1.png} \\
%Complex Stroma & & & \\
\parbox[t]{2mm}{\multirow{1}{*}{\rotatebox[x=-10in]{90}{\vspace{10pt}Immune Cells\hspace{-55pt}}}}&
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/15_0_3.png}&
\includegraphics[width=1.0in,height=1.0in, cfbox=green 3pt]{figs/colon_ret/15_1_3.png}&
\includegraphics[width=1.0in,height=1.0in, cfbox=green 3pt]{figs/colon_ret/15_2_3.png}&
\includegraphics[width=1.0in,height=1.0in, cfbox=green 3pt]{figs/colon_ret/15_3_3.png} \\
%Immune Cells & & & \\
\parbox[t]{2mm}{\multirow{1}{*}{\rotatebox[x=-10in]{90}{\vspace{10pt}Debris and Mucus\hspace{-63pt}}}}&
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/12_0_4.png}&
\includegraphics[width=1.0in,height=1.0in, cfbox=green 3pt]{figs/colon_ret/12_1_4.png}&
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/12_2_2.png}&
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/12_3_0.png} \\
%Debris and Mucus & & & \\
\parbox[t]{2mm}{\multirow{1}{*}{\rotatebox[x=-10in]{90}{\vspace{10pt}Mucosal Glands \hspace{-60pt}}}}&
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/0_0_5.png}&
\includegraphics[width=1.0in,height=1.0in, cfbox=green 3pt]{figs/colon_ret/0_1_5.png}&
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/0_2_4.png}&
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/0_3_4.png} \\
%Mucosal Glands & & & \\
\parbox[t]{2mm}{\multirow{1}{*}{\rotatebox[x=-10in]{90}{\vspace{10pt}Adipose Tissue\hspace{-60pt}}}}&
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/37_0_6.png}&
\includegraphics[width=1.0in,height=1.0in, cfbox=green 3pt]{figs/colon_ret/37_1_6.png}&
\includegraphics[width=1.0in,height=1.0in, cfbox=green 3pt]{figs/colon_ret/37_2_6.png}&
\includegraphics[width=1.0in,height=1.0in, cfbox=green 3pt]{figs/colon_ret/37_3_6.png} \\
%Adipose Tissue& & & \\
\parbox[t]{2mm}{\multirow{1}{*}{\rotatebox[x=-10in]{90}{\vspace{10pt}Background\hspace{-50pt}}}}&
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/11_0_7.png}&
\includegraphics[width=1.0in,height=1.0in, cfbox=green 3pt]{figs/colon_ret/11_1_7.png}&
\includegraphics[width=1.0in,height=1.0in, cfbox=green 3pt]{figs/colon_ret/11_2_7.png}&
\includegraphics[width=1.0in,height=1.0in, cfbox=green 3pt]{figs/colon_ret/11_3_7.png} \\
%Background & & & \\
\end{tabular}
}
}
}
\caption{A visualization of top 3 retrieval performance on colon cancer dataset without training on the target dataset. After training our model via ProxyNCA on the Weakly-labeled dataset (KimiaPath24), we compute the euclidean distance of image features with respect to the all the other images in target dataset. Correctly retrieved images (same class as query image) is highlighted with a green-box. Query image are selected randomly from the dataset.}
%first row image label 0 (normal)
%second row image lable 1 (cancer)
\label{fig:colonret}
\end{figure}
%%%%

\begin{table}[H]
\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{cccc} \hline
$N_c$ & $R$\% & Initialization/Method & Accuracy (\%) \\ \hline
12 & 2 & Random & 63.32 $\pm$ 2.56\\
  &  & Classification & \textbf{82.66 $\pm$ 2.89}\\
  &  & ProxyNCA & 82.48 $\pm$ 2.65\\  \hline
25 & 4 & Random & 65.94 $\pm$ 4.24\\
 &  & Classification & \textbf{87.32 $\pm$ 1.35}\\
 &  & ProxyNCA & 86.94 $\pm$ 1.87\\  \hline
50 & 9 & Random & 77.54 $\pm$ 2.08\\
 &  & Classification & 89.82 $\pm$ 1.56\\
 &  & ProxyNCA & \textbf{89.90 $\pm$ 1.35}\\  \hline
%62 & 11 & Random & 80.38\\
% &  & Classification & \textbf{90.72}\\
% &  & ProxyNCA & 90.62\\  \hline
100 & 18 & Random & 83.92 $\pm$ 0.97\\
 &  & Classification & 91.16 $\pm$ 1.13\\
 &  & ProxyNCA & \textbf{91.26 $\pm$ 1.04}\\ \hline
625 & 100 & Random & 89.58 $\pm$ 0.62\\
 &  & Classification & \textbf{92.70 $\pm$ 1.22}\\
 &  & ProxyNCA & 92.60 $\pm$ 0.95\\
%625 & 100 & RBF-SVM* \cite{kather2016multi}& 80.80 \\
 &  & RBF-SVM \cite{kather2016multi}& 87.40 \\
\hline
\end{tabular}
\bigskip
    \caption{Accuracy of our model trained with $R$\% of data in three different pre-trained settings on the CRC dataset. $N_c$ denotes the number of examples per class.  We compare our approach with  the best model in \cite{kather2016multi} which is a RBF-SVM model that uses 5 different concatenated features (Lower-order histogram, Higher-order histogram, Local Binary Patterns, Gray-Level Co-occurrence Matrix and Ensemble of Decision Trees).}
    \label{table:exp_1}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[h]
\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{cccc} \hline
$N_c$ & $R$\% & Initialization/Method & Accuracy (\%) \\ \hline
1,000 & 0.76 & Random & 79.37 $\pm$ 1.33 \\
 & & Classification & 85.29 $\pm$ 1.08\\
 & & ProxyNCA & \textbf{86.69 $\pm$ 0.46}\\  \hline
2,000 & 1.53 & Random & 81.26 $\pm$ 1.47\\
 & & Classification & 86.55 $\pm$ 1.29\\
 & & ProxyNCA & \textbf{87.38 $\pm$ 0.78}\\  \hline
3,000 & 2.29 & Random & 84.09 $\pm$ 1.24\\
 &  & Classification & 87.03 $\pm$ 0.62\\
 &  & ProxyNCA & \textbf{87.69 $\pm$ 0.72}\\ \hline
13,107 & 10 & Random & 88.47 $\pm$ 0.59\\
 &  & Classification & 89.64 $\pm$ 0.39\\
 &  & ProxyNCA & \textbf{89.77 $\pm$ 0.50}\\ \hline
131,072 & 100 & Random & 88.98 $\pm$ 1.06\\
 &  & Classification & 89.85 $\pm$ 0.64\\
 &  & ProxyNCA & \textbf{90.47 $\pm$ 0.59}\\
 &  & P4M\cite{veeling2018rotation} & 89.97\\
 %&  & Baseline\cite{teh:MIDLAbstract2019a} & 89.21 \\
 %&  & Pi\cite{teh:MIDLAbstract2019a} & 89.94 $\pm$ 0.34 \\
 &  & Pi+\cite{teh:MIDLAbstract2019a} & 90.36 $\pm$ 0.41\\
\hline
\end{tabular}
\bigskip
    \caption{Accuracy of our model trained with $R$\% of data in three different pre-trained settings on the PCam dataset. $N_c$ denotes the number of examples per class. We compare our approach to \cite{veeling2018rotation}, which uses a DenseNet with group convolutional layers and \cite{teh:MIDLAbstract2019a} which uses contrastive and self-perturbation loss together with cross entropy loss.
    }
    \label{table:exp_2}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%
\begin{figure}[H]
\centering
{\setlength{\tabcolsep}{2pt}
\scalebox{0.64}{ %0.64
\fbox{
\begin{tabular}{cc!{\vrule width 5pt}ccc}
&
\textbf{Query} & \textbf{Rank 1} & \textbf{Rank 2} & \textbf{Rank 3}\\
\parbox[t]{3mm}{\multirow{1}{*}{\rotatebox[x=-10in]{90}{\vspace{10pt}Tumour Epithelium\hspace{-65pt}}}}&
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/36_0_0.png}\ \ \ &
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/36_1_2.png}&
\includegraphics[width=1.0in,height=1.0in, cfbox=green 3pt]{figs/colon_ret/36_3_0.png}&
\includegraphics[width=1.0in,height=1.0in, cfbox=green 3pt]{figs/colon_ret/36_3_0.png} \\
%Tumour Epithelium & & & \\
\parbox[t]{2mm}{\multirow{1}{*}{\rotatebox[x=-10in]{90}{\vspace{10pt}Simple Stroma\hspace{-60pt}}}}&
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/7_0_1.png}&
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/7_1_2.png}&
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/7_2_2.png}&
\includegraphics[width=1.0in,height=1.0in, cfbox=green 3pt]{figs/colon_ret/7_3_1.png} \\
%Simple Stroma & & & \\
\parbox[t]{2mm}{\multirow{1}{*}{\rotatebox[x=-10in]{90}{\vspace{10pt}Complex Stroma\hspace{-60pt}}}}&
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/1_0_2.png}&
\includegraphics[width=1.0in,height=1.0in, cfbox=green 3pt]{figs/colon_ret/1_1_2.png}&
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/1_2_3.png}&
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/1_3_1.png} \\
%Complex Stroma & & & \\
\parbox[t]{2mm}{\multirow{1}{*}{\rotatebox[x=-10in]{90}{\vspace{10pt}Debris and Mucus\hspace{-63pt}}}}&
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/12_0_4.png}&
\includegraphics[width=1.0in,height=1.0in, cfbox=green 3pt]{figs/colon_ret/12_1_4.png}&
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/12_2_2.png}&
\includegraphics[width=1.0in,height=1.0in]{figs/colon_ret/12_3_0.png} \\
\end{tabular}
}
}
}
\caption{A visualization of top-3 retrieval performance on the CRC dataset with features trained on the weakly labeled dataset. Correctly retrieved images (same class as query image) are highlighted with a green-box. Query images are selected randomly from the dataset.}
%first row image label 0 (normal)
%second row image lable 1 (cancer)
\label{fig:colonret}
\end{figure}
%%%%

In Figure~\ref{fig:colonret}, we qualitatively show the retrieval performance on four different cells with features trained on weakly labeled data. We use the activation of the pre-trained embedding layer as image features. Retrieval is performed by computing the Euclidean distance between features of query images and features of all other images in the CRC dataset.
